Performing all-atom molecular dynamics simulations of intrinsically disordered proteins with replica exchange solute tempering

All-atom molecular dynamics (MD) computer simulations are a valuable tool for characterizing the conformational ensembles of intrinsically disordered proteins (IDPs). IDP conformational ensembles are highly heterogeneous and contain structures with many distinct topologies separated by large free-energy barriers. Sampling the vast conformational space of IDPs in explicit solvent all-atom MD simulations is extremely challenging, and enhanced sampling methods are generally required to obtain statistically meaningful descriptions of IDP conformational ensembles. Replica exchange solute tempering (REST) methods, where multiple coupled simulations of a system are performed in parallel with selectively modified potential energy functions, are a powerful approach for efficiently sampling the conformational space of IDPs. In this chapter, we demonstrate how to set-up, perform and analyze all-atom MD simulations of IDPs with REST enhanced sampling methods.

==> equations/REHT_exchange.tex <==
\begin{eqnarray}
    \begin{split}
        \left\{ {X_m,\,H_m\left( {X_m} \right),\,T_m} \right\} 	&\to \left\{ {X_n,\,H_m\left( {X_n} \right),T_m} \right\}\\ 
        \left\{ {X_n,\,H_n\left( {X_n} \right),\,T_n} \right\} 	&\to \left\{ {X_m,\,H_n\left( {X_m} \right),T_n} \right\},
    \end{split}
\end{eqnarray}

==> equations/epsilon_scaling.tex <==
% \begin{center}
%     \begin{equation}
      % $  \epsilon_{i}^{scaled}=\lambda_{n}\cdot \epsilon_i$ and $\epsilon_{OW}^{scaled} = \kappa_{n}^{2} * \epsilon_{OW}$
    % \label{eq:epsilon_scaling}
%     \end{equation}
% \end{center}

==> equations/kappa_scaling.tex <==
\begin{center}
    \begin{equation}
        \kappa_{n}=
        \begin{cases}
            1,  &n \leq 3 \\
            1+ 0.005(m-3),  &n > 3
        \end{cases}
    \label{eq:kappa_scaling}
    \end{equation}
\end{center}

==> equations/lambda_scaling.tex <==
\begin{center}
    \begin{equation} 
        \lambda_n = \frac{\beta_{n}}{\beta_{0}};\ \beta_{n}=\frac{1}{k_{B}T_{n}}\ for\ n=\{0,1,2,\ldots,n_{replica}\}
    \label{eq:lambda_scaling}     
    \end{equation}
\end{center}

==> equations/lj_potential.tex <==
\begin{center}
    \begin{equation}
        \begin{array}{ll}
            C^{(6)}_i &= 4\epsilon_i\sigma^6_i ; C^{(12)}_i = 4\epsilon_i\sigma^{12}_i \\
            C^{(6)}_{ij} &= \sqrt{C^{(6)}_i C^{(6)}_j}; C^{(12)}_{ij} = \sqrt{C^{(12)}_i C^{(12)}_j}\\
            E_{i,j}^{lj} &= \frac{C^{(12)}_{ij}}{r^{12}} -  \frac{C^{(6)}_{ij}}{r^{6}}
        \end{array}
    \label{eq:lj_potential}
    \end{equation}
\end{center}

==> equations/lj_potential_copy.tex <==
\begin{center}
    \begin{equation}
        \sqrt{\lambda_n}\cdot\kappa_n\cdot E_{i,OW}^{lj} = \sqrt{\lambda_n}\cdot \kappa_n \cdot 4 \cdot\epsilon_{i,OW}\Big[ \Big( \frac{\sigma_{i,OW}}{r}\big)^{12} -  \Big( \frac{\sigma_{i,OW}}{r}\big)^{6} \Big]
    \label{eq:lj_potential}
    \end{equation}
\end{center}

==> equations/reht_AR.tex <==
\begin{equation}
    {\Delta}_{{\boldsymbol{n,n+1}}}\left( {{{\mathrm{REHT}}}} \right) = - \left[ \begin{array}{l}(\beta _n\lambda _{\mathrm{n}} - \beta _{n+1}\lambda _{\mathrm{n+1}})\left[ {H_{pp}\left( {X_n} \right) - H_{pp}\left( {X_{n+1}} \right)} \right]\\ + \left( {\beta _n\sqrt {\lambda _{\mathrm{n}}} - \beta _m\sqrt {\lambda _{\mathrm{n+1}}} } \right)\left[ {H_{pw}\left( {X_n} \right) - H_{pw}\left( {X_{n+1}} \right)} \right]\\ + \left( {\beta _n - \beta _{n+1}} \right)\left[ {H_{ww}\left( {X_n} \right) - H_{ww}\left( {X_{n+1}} \right)} \right]\end{array} \right]
\end{equation}

==> equations/rest1_AR.tex <==
\begin{center}
    \begin{equation}
        \Delta_{n,n+1} = (\beta_{n}) - (\beta_{n+1})[(E_{pp}(X_{n+1}) + \frac{1}{2}E_{pw}(X_{n+1})) - (E_{pp}(X_{n}) + \frac{1}{2}E_{pw}(X_{n}))].
        \label{eq:rest1_AR}
    \end{equation}
\end{center}

==> equations/rest3_hamiltonian.tex <==
\begin{center}
    \begin{equation}
        E_{n}^{REST3}(X_{n}) = \lambda_{n} E_{pp}(X_{n}) + \sqrt{\lambda_{n}}\Big[ E_{pw}^{elec} + \kappa_n E_{pw}^{lj} \Big](X_{n}) +  E_{ww} (X_{n}).
        \label{eq:rest3_hamiltonian}
    \end{equation}
\end{center}

==> equations/thermodynamic_beta.tex <==
$\beta_{n}=\frac{1}{k_{B}T_{n}}\ for\ n=\{0,1,2,\ldots,n_{replica}\}$

==> equations/water_scaling.tex <==
\begin{center}
    \begin{equation}
        \begin{array}{ll}
            C^{(6),s}_{pw} =& \kappa_n \sqrt{\lambda_n} C^{(6)}_{pw}, \\ 
            C^{(12),s}_{pw} =& \kappa_n \sqrt{\lambda_n} C^{(12)}_{pw}, \\
            C^{(6),s}_{pp} =& \lambda_n C^{(6)}_{pw}, \\ 
            C^{(12),s}_{pp} =& \lambda_n C^{(12)}_{pw}, 
        \end{array}
    \label{eq:wat_scaling}
    \end{equation}
\end{center}

==> figures/lj_curves.tex <==
\begin{figure}
    \includegraphics[width=\textwidth]{./figures/Figure_a/fig_a.pdf}
    \caption{LJ potential for differing values of epsilon for a protein-protein atom pair (left) and protein-water atom pair (right). For protein-protein scaling the LJ potential well depth is only scaled by $\lambda_n$ for both REST2 and REST3. When scaling protein water interactions, the LJ potential well depth is scaled by either $\sqrt{\lambda_n}$ or $\kappa_n\sqrt{\lambda_n}$ for REST2 or REST3, respectively.}
    \label{fig:lj_curves}
\end{figure}

==> figures/vdw_figure.tex <==
\begin{figure}
    \includegraphics{./figures/Figure_a/fig_a.pdf}  
    \caption{Lj potential energy of paired atom types.}  
\end{figure}


==> tables/acc_ratio.tex <==

    \begin{table}[ht!]
        \centering
        \caption{Table showing the acceptance ratio between the replicas after 1$\mu$s of REST2 simulations.}
        \begin{tabular}{c | c | c }

        i & j & ACC\_R \\
        \hline
        0 & 1 & \num[round-mode=places,round-precision=3]{0.30945} \\
        \hline
        1 & 2 & \num[round-mode=places,round-precision=3]{0.317905} \\
        \hline
        2 & 3 & \num[round-mode=places,round-precision=3]{0.325348} \\
        % \hline
        % 3 & 4 & \num[round-mode=places,round-precision=3]{0.331818} \\
        \hline
        . & . & .\\ 
        . & . & .\\  
        . & . & .\\ 
        \hline
        8 & 9 & \num[round-mode=places,round-precision=3]{0.37185} \\
        \hline

        \end{tabular}
        \label{tab:acc_ratio_table}
        
    \end{table}


==> tables/vdw_noscaling_table.tex <==

    \begin{table}[ht!]
        \centering
        \caption{Table with $(\sigma_{ij}, \epsilon_{ij})$ showing the solvent interactions with itself and ions remain unaffected by the scaling factor $\kappa_{n}$.}
        \begin{tabular}{c | c c c }

        Atom types & OW$_{tip4pd}$ & NA$^{+}_{C22^{*}}$ & CL$^{-}_{C22^{*}}$ \\
        \hline
        OW$_{tip4pd}$ & (0.3165, 9.98989) & (0.279746, 0.442754)  & (0.360484, 0.791812)\\
        
        \hline
        \end{tabular}
        \label{tab:eps_noscale_table}
        
    \end{table}


==> tables/vdw_scaling_table.tex <==
\begin{table}[ht!]
    \centering
    \caption{Table showing the differences unscaled and the scaled $450K$ replica with REST2. Examples are shown for each type of parameter of the protein topology.}
    \begin{tabular}{c | c c c c c }

    Method & $T_{max}(K)$ & $\lambda$ & $\epsilon_{CA}$ & $\kappa$ & $\epsilon_{OW}$ \\
    \hline
    -- & 300 & 1.0 & 0.359824 & 1.0 & 0.998989 \\
    REST2 & 450 & 0.666667 & 0.239883 & 1.0 & 0.998989 \\

    ssREST3 & 450 & 0.666667 & 0.239883 & 1.1 & 1.20878 \\
    
    \hline
    \end{tabular}
    
    \label{tab:eps_table}
\end{table}
